Generalization of LRU Cache Replacement Policy with Applications to Video Streaming

Caching plays a crucial role in networking systems to reduce the load on the network and is commonly employed by content delivery networks (CDNs) in order to improve performance. One of the commonly used mechanisms, Least Recently Used (LRU), works well for identical file sizes. However, for asymmetric file sizes, the performance deteriorates. This paper proposes an adaptation to the LRU strategy, called gLRU, where the file is sub-divided into equal-sized chunks. In this strategy, a chunk of the newly requested file is added in the cache, and a chunk of the least-recently-used file is removed from the cache. Even though approximate analysis for the hit rate has been studied for LRU, the analysis does not extend to gLRU since the metric of interest is no longer the hit rate as the cache has partial files. This paper provides a novel approximation analysis for this policy where the cache may have partial file contents. The approximation approach is validated by simulations. Further, gLRU outperforms the LRU strategy for a Zipf file popularity distribution and censored Pareto file size distribution for the file download times. Video streaming applications can further use the partial cache contents to help the stall duration significantly, and the numerical results indicate significant improvements (32\%) in stall duration using the gLRU strategy as compared to the LRU strategy. Furthermore, the gLRU replacement policy compares favorably to two other cache replacement policies when simulated on MSR Cambridge Traces obtained from the SNIA IOTTA repository.

==> discuss_joint.tex <==
\section{Joint Popularity and File Size Distribution}\label{sec:dependence}
We now briefly consider the impact of the joint distribution of the popularity and file size on each of our performance metrics.
Modeling this joint distribution can be quite complicated.
In particular, specifying a probability measure such that the marginal distributions are Zipf for popularity and Pareto for file size while imposing a given correlation structure between the two is a nontrivial problem on its own.

In this section, we consider of the effect of strong positive and negative correlation between popularity and file size through simulation.
The system, as described in Section \ref{sec:videoStream}, is simulated with one major change.
In order to induce strong positive correlation we simply assign the highest popularities to the largest files and vice versa to induce negative correlation.
The system was then simulated for all of the combinations of parameters described in Table \ref{tab:paramDef} for both cases resulting in 384 cases for each.

Table \ref{tab:posvneg} presents a comparison of the positive and negative correlation cases for both the gLRU and LRU settings.
For each of the performance metrics described in Section \ref{sec:videoStream}, we present the average relative difference in performance positive vs. negative correlation (i.e. (positive metric - negative metric)/positive metric).
\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
Metric & gLRU & LRU \\
\hline \hline
$p_c$ & -.41     & -.47       \\
\hline
$p_m$ & 4.03	 & 2.16     \\
\hline
$T_w$ & 9.52     & 8.02 \\
\hline
$T_d$ & 4.99     & 4.28 \\
\hline
$p_d$ & 2.42         & 1.37     \\
\hline
\end{tabular}
\caption{Mean relative difference in performance for the positive vs. negative correlation setting. Value are computed as (positive correlation - negative correlation)/negative correlation for each metric of interest.}
\label{tab:posvneg}
\end{table}
The results show that the case of negative correlation vastly outperforms the case of positive correlation in both when employing either a gLRU or LRU replacement policy.
%In addition, our results indicate that positive correlation failed to result in better performance for any trial or performance metric.
%We see that the negative correlation results in a superior 
%
%The results indicated that over almost every metric negative correlation results in superior performance.
%While this is, indeed, an interesting result the particular reasons are not clear and the subject of future work.
This is because in the case of negative correlation, most popular files are smaller and thus more of them can be stored in the cache improving all the metrics as compared to when there is positive correlation. 

%It makes sense that, since the most popular files are smaller in the negative correlation case, then more of them can be stored in the cache.
%However, one would expect that the files not stored in the cache are much larger and would incur much higher delays on the off chance that they are selected.

In addition, we note that gLRU outperforms LRU in both the positive and negative correlation case.
In Table \ref{tab:posneg}, we present the mean relative performance improvement for gLRU vs LRU in all performance metrics of interest in both the correlation settings.
\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
Metric & Positive Correlation & Negative Correlation \\
\hline \hline
$p_c$ & .42     & .21        \\
\hline
$p_m$ & -.57 	&  -1.51    \\
\hline
$T_w$ & -.10    & -.82\\
\hline
$T_d$ & -.14    & -.69 \\
\hline
$p_d$ & -.16    & -.46     \\
\hline
\end{tabular}
\caption{Mean relative performance improvement of gLRU over LRU in the case of both positive and negative correlation for each of the performance metrics outlined in Section \ref{sec:videoStream}}
\label{tab:posneg}
\end{table}
While the results are much more pronounced in the case of negative correlation, it is clear that gLRU outperforms LRU in both correlation cases.
For a more granular look at the data see Appendix \ref{app:corrhist}.

